On the Opportunities of Large Language Models for Programming Process Data

Computing educators and researchers have used programming process data to understand how programs are constructed and what sorts of problems students struggle with. Although such data shows promise for using it for feedback, fully automated programming process feedback systems have still been an under-explored area. The recent emergence of large language models (LLMs) have yielded additional opportunities for researchers in a wide variety of fields. LLMs are efficient at transforming content from one format to another, leveraging the body of knowledge they have been trained with in the process. In this article, we discuss opportunities of using LLMs for analyzing programming process data. To complement our discussion, we outline a case study where we have leveraged LLMs for automatically summarizing the programming process and for creating formative feedback on the programming process. Overall, our discussion and findings highlight that the computing education research and practice community is again one step closer to automating formative programming process-focused feedback.

==> prompts/1-change-describer-prompt.tex <==
\begin{figure}[h!tbp]
\centering
\begin{example}{Prompt format for summarizing the programming process}

You are an introductory programming teaching assistant who is an expert in analyzing programming process data and an expert in summarizing how students construct their programs based on the programming process data  \circled{1}. You are studying how a student solved a programming problem by analyzing the programming process data \circled{2}.\\

Here's the handout for the programming problem:\\

\textcolor{blue}{<handout>} \circled{3} \\

The programming process data is described as a sequence of steps, where each step is numbered and each step has the assignment header and the code. The format of the data is as follows: \circled{4} \\

\#\#\#\#\# \\
Step: step identifier \\
\#\#\#\#\# \\
(the code state that the student had at this step) \\

As an extremely good introductory programming teaching assistant, summarize how the student constructed their program based on the following programming process data. Respond as if you were talking to the student. Only summarize the programming process data. Do not provide any suggestions or feedback. \circled{5} \\

\textcolor{blue}{<process data>} \circled{6}
\end{example}
\caption{Prompt format for summarizing the programming process. The prompt included (1) a description of the context and the persona, (2) the broader task, (3) the handout, (4) the format of the input data, (5) the explicit task instructions, and (6) the process data.}
\label{fig:process_summarization_prompt}
\end{figure}

==> sample-outputs/old-feedback-sample.tex <==

\begin{quote} % This is row 301 from the file
Reviewing your programming process from the initial steps to the final solution, you've shown consistent improvement and refined your approach to solving the problem efficiently. However, there are a few areas where further refinements could enhance both your code's performance and your programming technique. Here's a breakdown of suggestions based on your steps:\\

\textbf{General Observations Across Steps}\\

\begin{enumerate}
    \item \textbf{Variable Naming:} Your variable names have improved over time in terms of clarity, but ensure consistency and specificity in naming. For instance, \texttt{seedNumber} is an excellent choice, as it clearly denotes its purpose in the context of seeding the random number generator. Keep focusing on clear, descriptive names for improved code readability.
    \item \textbf{Import Statements:} You transitioned from a specific import statement (\texttt{from random import seed, randint}) to importing the whole \texttt{random} module. Both approaches are valid, but your final choice (\texttt{import random}) is typically more readable and makes it clear where functions like \texttt{random.seed()} and \texttt{random.randint()} are coming from. However, ensure you use this approach consistently across your program to avoid confusion or potential errors.
    \item \textbf{Loop Controls:} You've made efficient use of break statements to exit loops early, which is crucial for performance in this context. This technique, especially combined with your condition to stop the outer loop after finding 7 Fluky Numbers, demonstrates an understanding of controlling loop execution efficiently.
\end{enumerate}

\vspace{3mm}

\textbf{Specific Suggestions}\\


\begin{itemize}
    \item \textbf{Step 001 to Step 002:} Your early steps involved experimenting with the random module and starting to construct loops for factor checking. It's good practice to run small tests like these to ensure you understand how specific functions work. However, make sure to also plan out your solution's structure early on to guide these experiments.
    \item \textbf{Step 003:} You attempted to nest loops unnecessarily, which could potentially cause confusion or inefficiencies. Remember, nested loops should be used when each loop's iterations depend on the previous loop's state. For finding factors, a single loop can suffice.
    \item \textbf{Step 004 to Step 010:} You demonstrated an understanding of optimizing your solution by reducing the range for factor finding and implementing conditions to break loops early effectively. Continue refining these heuristics for efficiency, but also ensure they are justified and do not inadvertently skip potential solutions.
    \item \textbf{Final Implementation:} Your use of time measurement to report the execution duration is excellent for analyzing performance. Keep this practice for future projects to assess and improve the efficiency of your solutions.
\end{itemize}

\vspace{3mm}

\textbf{Additional Recommendations}\\

\begin{enumerate}
    \item \textbf{Commenting:} While your code is structured logically, adding comments to explain your thought process, especially why certain optimizations (like breaking the loop if \texttt{seedNumber >= 397}) were implemented, would be beneficial. This not just aids others in understanding your code, but it can help you as well when revisiting your own work.
    \item \textbf{Testing and Validation:}  Implement a step dedicated to verifying the correctness of your found Fluky Numbers. While the output meets the expected count, ensuring the accuracy of these numbers through assert statements or other means would solidify your solution's correctness.
    \item \textbf{Performance Analysis:} Although you've done well to measure and print the total running time, consider digging deeper into which parts of your program consume the most time and why. This could lead to discovering more sophisticated optimization opportunities.
\end{enumerate}

\vspace{3mm}

Keep exploring and refining your approach with these suggestions in mind. Your journey from the initial attempt to the final solution showcases your ability to learn and improve, which is commendable.    
\end{quote}
